Boosting Adversarial Robustness using Feature Level Stochastic Smoothing

Advances in adversarial defenses have led to a significant improvement in the robustness of Deep Neural Networks. However, the robust accuracy of present state-ofthe-art defenses is far from the requirements in critical applications such as robotics and autonomous navigation systems. Further, in practical use cases, network prediction alone might not suffice, and assignment of a confidence value for the prediction can prove crucial. In this work, we propose a generic method for introducing stochasticity in the network predictions, and utilize this for smoothing decision boundaries and rejecting low confidence predictions, thereby boosting the robustness on accepted samples. The proposed Feature Level Stochastic Smoothing based classification also results in a boost in robustness without rejection over existing adversarial training methods. Finally, we combine the proposed method with adversarial detection methods, to achieve the benefits of both approaches.

==> tables/IN_bu.tex <==
\begin{table*}[]
\caption{ImageNet-$100$: Performance (\%) of models under an ensemble of 4 attacks : PGD, APGD-CE, APGD-DLR, SQUARE. FC denotes the set of samples which are always correctly classified and accepted for all attacks. FW denotes the set of samples which are accepted and incorrectly classified by at least one of the attacks. MPR denotes the max $\%$ rejected samples.}
\label{table:imagenet}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc}
\toprule
\multicolumn{1}{l|}{}             & $Acc_{nat, NS}\uparrow$ & $Acc_{adv, NS}\uparrow$ & $Acc_{nat, 0\%}\uparrow$ & $Acc_{nat, 10\%}\uparrow$ & $Acc_{adv, 0\%}\uparrow$ & $Acc_{adv, 10\%}\uparrow$ & $Err_{adv, 10\%}\downarrow$ & FC$\uparrow$          & FW$\downarrow$          & MPR \\
\midrule
PGD(Conf.)              & 59.97                 & 28.46                 & 59.97                & 73.68  & 28.46                & 30.19                 & 65.88                 & 28.26                & 65.88                & 16.0                      \\
Trades(Conf.) & 62.33                 & 31.72                    & 62.33 & 77.42                 & 31.72                  & 43.76                 & 38.72                 & 30.14                & 38.72                & 41.98                   \\
\textbf{Ours}                  & 56.21                 &  31.48 & 56.46                & 78.72                 &32.60  &  47.19 &  31.40 & 28.06 &31.40  & 58.84   \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/adaptive_imagenet.tex <==
\begin{table}[]
\caption{\textbf{ImageNet-$100$}: Performance (\%) of the proposed model against various adaptive attacks. MPR denotes the maximum percentage rejected samples.}
\label{table:in_adaptive}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cccc}
\toprule
& \multicolumn{1}{c}{\textbf{$Acc_{adv, 0\%}\uparrow$}} & \multicolumn{1}{c}{\textbf{$Acc_{adv, 10\%}\uparrow$}} & \multicolumn{1}{c}{\textbf{$Err_{adv, 10\%}\downarrow$}} & \multicolumn{1}{c}{MPR} \\
\midrule
A1: FA (KL, targ)          & 41.20                                     & 56.70                                      & 22.60                                      & 59.10                                        \\
A2: FA (MSE, targ)         & 41.00                                       & 52.43                                     & 25.40                                      & 60.10                                        \\

A5: FA (MSE + min var, targ) & 40.80                                     & 54.05                                     & 25.90                                      & 61.09     \\
\midrule
RA1: Max entropy                 & 54.20                                     & 87.37                                     & 5.20                                       & 58.80                                        \\
RA2: Max entropy + Min CE       & 53.80                                     & 87.77                                     & 5.00                                         & 59.10                                        \\

\bottomrule
\end{tabular}}
\end{table}


==> tables/cifar_2.tex <==
\begin{table}[]
\caption{\textbf{CIFAR-$10$}: Performance (\%) of models under an ensemble of 5 attacks : PGD, APGD-CE, APGD-DLR, FAB, SQUARE.}
\label{table:cifar_2}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
               & \multicolumn{3}{c|}{$Acc_{nat}$}                                         & \multicolumn{3}{c}{$Acc_{adv}$}                \\
               \cmidrule(l){2-7}
               & No Samp.$\uparrow$ & $0\%$ rej.$\uparrow$ & $10\%$ rej.$\uparrow$ & No Samp.$\uparrow$ & $0\%$ rej.$\uparrow$ & $10\%$ rej.$\uparrow$ \\
\midrule
PGD (Conf)     & \textbf{84.37}                 & \textbf{84.37}                & 91.94                 & 44.40                  & 44.40                & 52.31                 \\
TRADES  (Conf) &  80.15 & 76.53 & 83.28  & 45.32                 & 45.32                & 56.61                 \\
\textbf{Ours}           & 80.20                 & 80.50                 & \textbf{91.63}                 & \textbf{47.48}                 & \textbf{51.11}                & \textbf{62.3}                 \\
\bottomrule
\end{tabular}}
\end{table}

==> tables/cifar_3.tex <==
\begin{table*}[]
\caption{\textbf{CIFAR-$10$}: Accuracy (\%) of models under individual attacks : PGD, APGD-CE, APGD-DLR, FAB, SQUARE. Worst case accuracy($\%$) across all attacks is also reported. For each attack, accuracy with $0\%$ rejection and $10\%$ rejection are reported.}
\label{table:cifar_3}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|c}
\toprule
\multicolumn{1}{l}{}         & \multicolumn{2}{|c}{PGD}                                  & \multicolumn{2}{|c}{APGD-CE}                              & \multicolumn{2}{|c}{APGD-DLR}                             & \multicolumn{2}{|c}{FAB}                                  & \multicolumn{2}{|c}{SQUARE}                               & \multicolumn{1}{|c}{ALL}                                  \\
\cmidrule(l){2-12}
\multicolumn{1}{l}{}         & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} &  \multicolumn{1}{|l}{~$Acc_{10\%}\uparrow$~} \\
\midrule
PGD (Conf. thresh)     & 46.21                      & 52.46                       & 45.63                      & 58.45                       & 47.32                      & 67.31                       & 45.52                      & 86.27                       & 53.42                      & 85.67                                            & 51.69                       \\
TRADES  (Conf. thresh) & 48.57                      & 59.85                       & 47.29  & 59.89   & 47.13                      & 64.27                       & 46.7                       & 71.83                       & 52.3                       & 75.91                                            & 56.61                       \\
PGD (Noise Sampling)               & 50.1                       & 54.58                       & 53.72                      & 60.97                       & 57.33                      & 67.54                       & 68.57                    & 77.79                       & 68.65                    & 78.53                       &         51.63                       \\
TRADES (Noise Sampling)            & 50.38                      & 55.58                       & 54.17                      & 61.8                        & 54.12                      & 62.73                       & 64.36                      & 72.87                       & 64.52                      & 72.24                       &         50.83                       \\
PGD-Rice (Conf. thresh)            & 50.81 & 62.29 & 50.15 & 70.31 & 49.17 & 70.67 & 47.44 & 72.71 & 53.45 & 76.83 & 58.25 \\
PNI-W (Noise sampling)         & 35.71 & 35.9  & 42.66 & 46.78 & 45.71 & 64.81 & 84.71 & 92.57 & 84.38 & 92.99 & 34.69 \\
Trades+RS (Noise sampling) & 48.81 & 53.75 & 50.58 & 58.37 & 49.84 & 59.04 & 64.48 & 72.88 & 62.57 & 72.42 & 49.28 \\
RS Std. train (Noise sampling)      & 20.81 & 18.66 & 26.67 & 24.26 & 44.18 & 49.82 & 82.27 & 88.35 & 78.2  & 84.92 & 16.17 \\

\textbf{Ours}                   & 56.48                      & 71.49                       & 60.03                      & 79.12                       & 57.19                      & 74.02                       & 67.59                      & 85.83                       & 69.02                      & 86.76                                            & \textbf{62.3}         \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/cifar_3_backup.tex <==
\begin{table*}[]
\caption{\textbf{CIFAR-$10$}: Accuracy (\%) of models under individual attacks : PGD, APGD-CE, APGD-DLR, FAB, SQUARE. Worst case accuracy($\%$) across all attacks is also reported. For each case, accuracy with no rejection and $10\%$ rejection is reported.}
\label{table:cifar_3}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc|cc}
\toprule
\multicolumn{1}{l}{}         & \multicolumn{2}{|c}{PGD}                                  & \multicolumn{2}{|c}{APGD-CE}                              & \multicolumn{2}{|c}{APGD-DLR}                             & \multicolumn{2}{|c}{FAB}                                  & \multicolumn{2}{|c}{SQUARE}                               & \multicolumn{2}{|c}{ALL}                                  \\
\cmidrule(l){2-13}
\multicolumn{1}{l}{}         & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} & \multicolumn{1}{|l}{~$Acc_{0\%}\uparrow$~} & \multicolumn{1}{l}{~$Acc_{10\%}\uparrow$~} \\
\midrule
PGD (Conf. thresh)     & 46.21                      & 52.46                       & 45.63                      & 58.45                       & 47.32                      & 67.31                       & 45.52                      & \textbf{86.27}                       & 53.42                      & 85.67                       & 44.4                       & 51.69                       \\
TRADES  (Conf. thresh) & 48.57                      & 59.85                       & 47.29  & 59.89   & 47.13                      & 64.27                       & 46.7                       & 71.83                       & 52.3                       & 75.91                       & 45.32                      & 56.61                       \\
PGD (Noise Sampling)               & 50.1                       & 54.58                       & 53.72                      & 60.97                       & 57.33                      & 67.54                       & \textbf{68.57}                    & 77.79                       & 68.65                    & 78.53                       &        & 51.63                       \\
TRADES (Noise Sampling)            & 50.38                      & 55.58                       & 54.17                      & 61.8                        & 54.12                      & 62.73                       & 64.36                      & 72.87                       & 64.52                      & 72.24                       &        & 50.83                       \\

\textbf{Ours}                   & \textbf{56.48}                      & \textbf{71.49}                       & \textbf{60.03}                      & \textbf{79.12}                       & \textbf{57.19}                      & \textbf{74.02}                       & 67.59                      & 85.83                       & \textbf{69.02}                      & \textbf{86.76}                       & \textbf{51.11}                      & \textbf{62.3}         \\
\bottomrule
\end{tabular}}
\end{table*}

==> tables/cifar_bb_pgd.tex <==
\begin{table}[]
\caption{\textbf{CIFAR-$10$}: Accuracy (\%) of models against PGD $7$-step Black-Box attack. Attack source is a normally trained model of the same architecture.}
\label{table:cifar_bb_pgd}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cc|cc|c}
\toprule
\multicolumn{1}{l|}{} & $Acc_{nat,0\%}\uparrow$               & $Acc_{nat,10\%}\uparrow$              & $Acc_{adv,0\%}\uparrow$ &$Acc_{adv,10\%}\uparrow$ & $Err_{adv,10\%}\downarrow$ \\
\midrule
PGD (Conf)            & 84.37                           & 91.94                     & 82.75       & 90.38        & 7.85                             \\
TRADES (Conf)        & 80.15                           & 88.45 & 78.47       & 86.94        & 9.45                             \\
PGD (Noise)    & 81.27                           & 89.46 & 79.59       & 85.82        & 12.14                            \\
TRADES (Noise) & 76.53                           & 83.28 & 74.90        & 80.98        & 16.26                            \\
\textbf{Ours}           & 80.50                            & 91.63                     & 78.91       & 90.26        & 7.33         \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/cifar_new.tex <==
\begin{table}[]
\caption{\textbf{CIFAR-$10$}: Accuracy (\%) of models under attacks with varying number of steps and restarts. Accuracy with no rejection and $10\%$ rejection is reported for each attack.}
\label{table:cifar_4}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
                & $Acc_{0\%}\uparrow$                                & $Acc_{10\%}\uparrow$                                & $Acc_{0\%}\uparrow$                                 & $Acc_{10\%}\uparrow$                                 & $Acc_{0\%}\uparrow$                        & $Acc_{10\%}\uparrow$ \\
                \midrule
No. of steps    & 100                                     & 100                                      & 1000                                     & 1000                                      &     100                            &                      100            \\

No. of restarts & 1                                       & 1                                        & 1                                        & 1                                         & 10                              & 10                               \\
\midrule
\midrule
PGD             & 42.9                                    & 49.69                                    & 42.8                                     & 49.13                                     & 42.8                            & 48.52                            \\
TRADES          & 44.6                                    & 53.97                                    & 44.6                                     & 54.12                                     & 44.5                            & 53.27                            \\
\textbf{Ours}            &   48.7                                      &          61.48                                &         48.5                                 &                                61.61           &   46.1                              & 52.6  \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/errata.tex <==
\begin{table}[h]
\caption{\textbf{Errata} : This table contains the corrections to typographical errors in the main paper.}
\label{table:errata}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|l|l}
\toprule
\textbf{Reference} & \textbf{Error}                  & \textbf{Correction}             \\
\midrule
\midrule
 & In order to assist the rejection of   & In order to assist the rejection of strong   \\
L305& strong adversaries, we minimize &adversaries, we maximize $KL_3$ (L-8 in \\
&$KL_3$ (L-8 in Algo.1) & Algo.1) \\
\midrule
Eq. 7 & $Acc_{adv,10\%} = \frac{|FC|}{|FC|+|FW|}$ & $Acc_{adv,10\%} = \frac{|FC|}{|FC|+|FW|} \cdot 100$ \\
\midrule
L447      & MR (Maximum Rejection) & MPR (Maximum Percentage Rejection) \\

\midrule
Eq. 8     & MR                     & MPR                               \\
\midrule
Eq. 9     & $Acc_{adv,10\%} = \frac{|FW|}{|X|}$              & $Err_{adv,10\%} = \frac{|FW|}{|\mathcal{X}|}\cdot100$   \\
\midrule
Table 1,  & FW denotes the set of samples  & FW denotes the set of samples which   \\  
Table 5     &   which are  rejected by at least             &  are accepted and incorrectly classified \\
caption    & one of the attacks.  &  by at least one of the attacks.  \\
\midrule
 & ImageNet-$100$: Performance (\%)    & ImageNet-$100$: Performance (\%) of  \\
Table 5  & of models under an ensemble of & models under an ensemble of 4 attacks \\
caption & 5 attacks: PGD, APGD-CE,   & PGD, APGD-CE, APGD-DLR, \\
& APGD-DLR, FAB, SQUARE. & SQUARE. \\
\midrule
Table 5 & $Err_{adv, 10\%}\uparrow$   & $Err_{adv, 10\%}\downarrow$ \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/imagenet_1.tex <==
\begin{table*}[]
\caption{ImageNet-$100$: Performance (\%) of models under an ensemble of 4 attacks : PGD, APGD-CE, APGD-DLR, SQUARE. FC denotes the set of samples which are always correctly classified and accepted for all attacks. FW denotes the set of samples which are accepted and incorrectly classified by at least one of the attacks. MPR denotes the max $\%$ rejected samples.}
\label{table:imagenet}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|c|cc|cc|cc|cc}
\toprule
\multicolumn{1}{l|}{}             & $Acc_{nat, NS}\uparrow$ &  $Acc_{nat, 0\%}\uparrow$ & $Acc_{nat, 10\%}\uparrow$ & $Acc_{adv, 0\%}\uparrow$ & $Acc_{adv, 10\%}\uparrow$ & $Err_{adv, 10\%}\downarrow$ & FC$\uparrow$          & FW$\downarrow$          & MPR$\downarrow$ \\
\midrule
PGD(Conf.)              & 59.97                                  & 59.97                &  73.68 & 28.46& 30.19                 & 65.88                 & 28.26                & 65.88                & 16                      \\
Trades(Conf.) & 62.33                                     & 62.33 & 77.42                 & 31.72                  & 43.76                 & 38.72                 & 30.14                & 38.72                & 41.98                   \\
\textbf{Ours}                  & 56.21                 &    56.46                & 78.72                 &32.6  &  47.19 &  31.4 & 28.06 &31.4  & 58.84   \\
\bottomrule
\end{tabular}}
\end{table*}


==> tables/imagenet_bb_fgsm.tex <==
\begin{table}[]
\caption{\textbf{ImageNet-$100$}: Accuracy (\%) of models against FGSM Black-Box attack. Attack source is a normally trained model of the same architecture.}
\label{table:in_bb_fgsm}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cc|cc|c}
\toprule
\multicolumn{1}{l|}{} & $Acc_{nat,0\%}\uparrow$               & $Acc_{nat,10\%}\uparrow$              & $Acc_{adv,0\%}\uparrow$ &$Acc_{adv,10\%}\uparrow$ & $Err_{adv,10\%}\downarrow$ \\
\midrule
PGD (Conf)           & 59.97       & 73.68        & 57.50        & 60.42        & 37.40         \\
TRADES (Conf)        & 62.33       & 77.42        & 61.20        & 74.00           & 19.00           \\
\textbf{Ours}        & 56.46       & 78.72        & 55.80        & 77.21        & 13.40          \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/in_restarts.tex <==
\begin{table}[]
\caption{\textbf{ImageNet-$100$}: Accuracy (\%) of models under attacks with varying number of steps and restarts. Accuracy with no rejection and $10\%$ rejection is reported for each attack.}
\label{table:in_restarts}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\toprule
                & $Acc_{0\%}\uparrow$                                & $Acc_{10\%}\uparrow$                                & $Acc_{0\%}\uparrow$                                 & $Acc_{10\%}\uparrow$                                 & $Acc_{0\%}\uparrow$                        & $Acc_{10\%}\uparrow$ \\
                \midrule
No. of steps    & 100                                     & 100                                      & 1000                                     & 1000                                      &     100                            &                      100            \\

No. of restarts & 1                                       & 1                                        & 1                                        & 1                                         & 10                              & 10                               \\
\midrule
\midrule
PGD (Conf)             & 28.60                    & 30.08                   & 28.22                    & 29.97                    & 28.50                   & 29.86                  \\
TRADES (Conf)         & 31.30                    & 42.75                   & 31.46                    & 42.85                    & 31.20                   & 41.77                  \\
\textbf{Ours}            & \textbf{33.80}                    & \textbf{47.60}                    & \textbf{32.30}                     & \textbf{46.05}                    & \textbf{33.40}                   & \textbf{46.73}      \\
\bottomrule
\end{tabular}}
\end{table}


==> tables/mt.tex <==
\begin{table*}[]
\caption{\textbf{Targeted and Untargeted Max-Margin based attacks}: Accuracy (\%) of models against (a) Ensemble of 5 attacks (PGD-$100$, APGD-CE, APGD-DLR, FAB, Square) (b) Untargeted attack with Maximum-margin objective (c) MultiTargeted attack \cite{gowal2019alternative}}
\label{table:mt}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{c|l|cc|cc|cc}
\toprule
\multirow{2}{*}{Dataset}      & \multirow{2}{*}{Model} & \multicolumn{2}{|c|}{Ensemble of 5 attacks}                    & \multicolumn{2}{c|}{Max-Margin attack} & \multicolumn{2}{c}{MultiTargeted attack}  \\
\cmidrule(l){3-8}
      &  & $Acc_{adv,0\%}\uparrow$ &$Acc_{adv,10\%}\uparrow$                    & $Acc_{adv,0\%}\uparrow$ &$Acc_{adv,10\%}\uparrow$       & $Acc_{adv,0\%}\uparrow$ &$Acc_{adv,10\%}\uparrow$       \\
\midrule

\multirow{3}{*}{CIFAR-10}     & PGD (Conf)           & 42.90                   & 49.69                  & 42.90          & 45.42          & 42.60            & 44.80            \\
                              & TRADES (Conf)~~~~~~~        & 44.60                   & 53.97                  & 45.70          & 49.01          & 44.50            & 48.52           \\
                              & \textbf{Ours}        & \textbf{49.30}                   & \textbf{65.71}                  & \textbf{47.60}          & \textbf{54.54}          & \textbf{46.20}            & \textbf{51.60}            \\
\midrule
\multirow{3}{*}{~~~ImageNet-100~~~} & PGD (Conf)           & 28.60                   & 30.08                  & 27.50          & 28.54          & 27.40            & 27.64           \\
                              & TRADES (Conf)        & 31.30                   & 42.75                  & 31.20          & 33.44          & 31.20            & 32.79           \\
                              & \textbf{Ours}        & \textbf{33.80}                   & \textbf{47.60}                   & \textbf{33.00}            & \textbf{39.14}          & \textbf{32.00}              & \textbf{37.24}    \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/pgd_restarts.tex <==
\begin{table}[]
\caption{\textbf{Random Restarts}: Accuracy (\%) of the proposed model against PGD-$50$ step attack without sampling during test time ($Acc_{adv, NS}$). The proposed model is stable across multiple restarts.}
\label{table:cifar_1}
\vspace{-0.0cm}
\setlength\tabcolsep{3pt}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{l|ccc}
\toprule
& \multicolumn{3}{c}{$Acc_{adv, NS}$~($\%$)} \\
\cmidrule(l){2-4}
         & \multicolumn{1}{l}{~~Single run$\uparrow$} & \multicolumn{1}{l}{$100$ restarts$\uparrow$} & \multicolumn{1}{l}{$1000$ restarts$\uparrow$} \\
         \midrule
CIFAR-$10$ & 56.6                          & 55.2                             & 55.1                              \\
ImageNet-$100$~~~ & 35.6                          & 35.3                             & 35.3        \\
\bottomrule
\end{tabular}}
\end{table}
